Judge as A Judge: Improving the Evaluation of Retrieval-Augmented Generation through the Judge-Consistency of Large Language Models

Retrieval-Augmented Generation (RAG) has proven its effectiveness in alleviating hallucinations for Large Language Models (LLMs). However, existing automated evaluation metrics cannot fairly evaluate the outputs generated by RAG models during training and evaluation. LLM-based judgment models provide the potential to produce high-quality judgments, but they are highly sensitive to evaluation prompts, leading to inconsistencies when judging the output of RAG models. This paper introduces the Judge-Consistency (ConsJudge) method, which aims to enhance LLMs to generate more accurate evaluations for RAG models. Specifically, ConsJudge prompts LLMs to generate different judgments based on various combinations of judgment dimensions, utilize the judge-consistency to evaluate these judgments and select the accepted and rejected judgments for DPO training. Our experiments show that ConsJudge can effectively provide more accurate judgments for optimizing RAG models across various RAG models and datasets. Further analysis reveals that judgments generated by ConsJudge have a high agreement with the superior LLM. All codes are available at https://github.com/OpenBMB/ConsJudge.

==> figure/eight_prompt.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{ 
\begin{tabular}{|l|}
\hline
\rowcolor{gray!8} \textbf{\textit{Dimensions Descriptions}} \\ 
\hline
\textbf{Hallucination}: Hallucination refers to the presence of information in the option that contradicts ground truth, \\
it is an incorrect answer to the question.\\
\textbf{Completeness}: Completeness refers to whether the choice contains as complete information as possible \\
from the ground truth. it did not fully answer the question correctly.\\
\textbf{Coherence}: coherence refers to whether the choice is logically coherent and whether the language between \\each sentence is fluent.\\
\textbf{Semantic Consistency}: Semantic Consistency refers to whether the choice is semantically consistent with \\the ground truth, rather than just having lexical repetition.\\

\hline
\rowcolor{gray!8} \textbf{\textit{Prompt}} \\
\hline
You are an excellent evaluation 
expert. Please select the best answer and the worst answer from four choices \\based on the 
ground truth and the query from the \{\textbf{\textit{Name of the hybrid evaluation aspects.}}\} aspect. \\ 
\{\textbf{\textit{Here is the descriptions of the hybrid evaluation aspects.}}\} \\
Note: your result format must strictly be "COT:\{.there 
is your analysis\}. \\Answer : Best answer:\{a choice 
must be one of[A,B,C,D]\}.\\
Worst answer :\{a choice must be one of[A, B, C, D]\}".\\ Output the content of COT first and 
then output the Answer.\\
Here is the query:\{query\}, Here is the ground truth:\{Ground Truth\}\\
Here is the A choice:\{choiceA\}, Here is the B choice:\{choiceB\},\\
Here is the C choice:\{choiceC\}, Here is the D choice:\{choiceD\}. \\
Result: \\
\hline
\end{tabular}
}
\caption{The Prompts of the \method{}.}
\label{table1:eightprompt}
\end{table*}




% \hline
% \rowcolor{gray!8} \textbf{\textit{Prompt 2}}\\
% \hline
% ... from the Completeness aspect. ... \\
% \hline
% \rowcolor{gray!8} \textbf{\textit{Prompt 3}}\\
% \hline
% ... from the \textbf{\textit{Coherence}} aspect. ... \\
% \hline
% \rowcolor{gray!8} \textbf{\textit{Prompt 4}}\\
% \hline
% ... from the \textbf{\textit{Semantic Consistency}} aspect. ... \\
% \hline
% \rowcolor{gray!8} \textbf{\textit{Prompt 5}}\\
% \hline
% ... from the \textbf{\textit{Hallucination and Completeness}} aspects. ... \\
% \hline
% \rowcolor{gray!8} \textbf{\textit{Prompt 6}}\\
% \hline
% ... from the \textbf{\textit{Coherence and Semantic Consistency}} aspects. ... \\
% \hline
% \rowcolor{gray!8} \textbf{\textit{Prompt 7}}\\
% \hline
% ... from the \textbf{\textit{Hallucination, Completeness and Semantic Consistency}} aspects. ... \\
% \hline
% \rowcolor{gray!8} \textbf{\textit{Prompt 8}}\\
% \hline
% ... from the \textbf{\textit{Hallucination, Completeness, Coherence and Semantic Consistency}} aspects. ... \\

==> table/ablation_n_3.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\hline
\multirow{1}{*}{\textbf{Reward model}} & \textbf{NQ} & \textbf{HotpotQA} & \textbf{TriviaQA} & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Avg.}}}\\
\hline
Raw Metric & 45.12 & 31.30& 79.12 & 51.85\\ \hline
\multicolumn{5}{l}{\textit{Llama3-8B}}\\
\hdashline
\method{} &  46.60 & \textbf{32.23} & \textbf{79.77}  & \textbf{52.87}\\
w/o Consistency & \textbf{47.06} & 31.88 & 79.12 & 52.69\\
w/o Query &  46.49 & 31.38 & 78.97 & 52.28\\
w/o Ground Truth &  46.18 & 31.45 & 79.21 & 52.28\\ 

\hline
\multicolumn{5}{l}{\textit{Qwen2.5-14B}}\\
\hdashline
\method{} &  \textbf{47.16} & \textbf{31.91} & \textbf{79.53} & \textbf{52.87}\\
w/o Consistency & 46.85 & 30.95 & 79.21 & 52.34\\
w/o Query  & 46.00	& 30.05 & 79.31 & 51.79\\
w/o Ground Truth & 46.74 & 31.76 & 79.32 & 52.61\\
\hline
\end{tabular}
}
\caption{Ablation Study. We use MiniCPM-2.4B to implement the RAG model.}

\label{table1:ablation}  % 设置表格的标签
\end{table}

==> table/overall_n_3.tex <==

\begin{table*}[ht]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|cccccccc}
\hline
%第一组
 % \textbf{Generator} & \textbf{Reward} &  \textbf{NQ} & \textbf{HotpotQA} & \textbf{TriviaQA} & \textbf{T-REx} & \textbf{ASQA} & \textbf{MARCOQA} & \textbf{WoW} & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Avg.}}}\\ 
 \multirow{2}{*}{\textbf{Generator}} & \multirow{2}{*}{\textbf{Reward}} & \textbf{NQ} & \textbf{HotpotQA} & \textbf{TriviaQA} & \textbf{T-REx} & \textbf{ASQA} & \textbf{MARCOQA} & \textbf{WoW} & \multirow{2}{*}{\textbf{Avg.}} \\ 
& & (acc) & (acc) & (acc) & (acc) & (str-em) & (llm) & (llm) & \\ 

% \cmidrule(lr){2-5} \cmidrule(lr){6-6} \cmidrule(lr){7-8} \
% Evaluation Metrics & \multicolumn{4}{c}{\textbf{Accuracy}} & \multicolumn{1}{c}{\textbf{Str EM}} & \multicolumn{2}{c}{\textbf{LLM}}\\

\hline
%\multirow{10}{*}{\shortstack{\textbf{MiniCPM}\\(2.4B)}}& \multicolumn{9}{c}{\textit{\textbf{Raw Metric\rlap{$\text{}^{\dagger}$}}}}\\\cline{2-10}
\multirow{7}{*}{\shortstack{\textbf{MiniCPM}\\(2.4B)}} & Raw Metric\rlap{$\text{}^{\dagger}$} & 45.12	& 31.30	& 79.12	&  32.46 & 35.44 & 88.42 & 87.76 & 57.09\\  \cdashline{2-10}
%& \multicolumn{9}{c}{\textit{\textbf{Llama3-8B}}}\\\cline{2-10}
    & Llama3-8B&  \textbf{47.34}	& 31.83 & 79.41	& 29.40	& 36.82	& 90.47	& 90.52 & 57.97\\
& w/ SFT &  46.84 & 31.34 & 79.06 & 27.20 & 37.04 & 91.26 & 90.24	& 57.57\\
&w/ \method{} &  46.60\rlap{$\text{}^{\dagger}$}	& \textbf{32.23}\rlap{$\text{}^{\dagger}$}	& \textbf{79.77}\rlap{$\text{}^{\dagger}$}	& \textbf{29.40}	& \textbf{37.12}\rlap{$\text{}^{\dagger}$}	& \textbf{91.35}\rlap{$\text{}^{\dagger}$}	& \textbf{91.24}\rlap{$\text{}^{\dagger}$}	& \textbf{58.24}
\\\cdashline{2-10}
%& \multicolumn{9}{c}{\textit{\textbf{Qwen2.5-14B}}}\\\cline{2-10}
& Qwen2.5-14B & 46.77 & 31.66 & \textbf{79.86} & 26.74 & 36.80 & 90.03 & 88.84 & 57.24\\
& w/ SFT &  46.98 & 31.76 & 79.14 & 32.38 & 36.88	& 90.57	& 89.92 & 58.23\\
& w/ \method{} &  \textbf{47.16}\rlap{$\text{}^{\dagger}$} & \textbf{31.91}\rlap{$\text{}^{\dagger}$} & 79.53\rlap{$\text{}^{\dagger}$} & \textbf{34.04}\rlap{$\text{}^{\dagger}$} & \textbf{38.35}\rlap{$\text{}^{\dagger}$} & \textbf{91.12}\rlap{$\text{}^{\dagger}$} & \textbf{90.04}\rlap{$\text{}^{\dagger}$} & \textbf{58.88}\\

\hline
%\multirow{6}{*}{\shortstack{\textbf{Llama3}\\(8B)}}& \multicolumn{9}{c}{\textit{\textbf{Raw Metric\rlap{$\text{}^{\dagger}$}}}}\\\cline{2-10}
\multirow{4}{*}{\shortstack{\textbf{Llama3}\\(8B)}} & Raw Metric\rlap{$\text{}^{\dagger}$} & 47.69 	& 33.22	& 84.55	&  30.22 & 40.69 & 89.36 & 84.30 & 58.58\\ \cdashline{2-10}
%& \multicolumn{9}{c}{\textit{\textbf{Llama3-8B}}}\\\cline{2-10}
& Llama3-8B&  46.67	& 33.54  & 85.82 & \textbf{42.18} & 41.65	& 90.18	& 86.43 & 60.92\\
& w/ SFT &  48.33 & 36.25 & \textbf{87.16} & 42.00 & \textbf{42.10} & 90.92 & 86.78 & 61.93\\
&w/ \method{}  & \textbf{48.54}\rlap{$\text{}^{\dagger}$} & \textbf{36.45}\rlap{$\text{}^{\dagger}$}	& 86.97\rlap{$\text{}^{\dagger}$} & 41.46\rlap{$\text{}^{\dagger}$}	& 41.78\rlap{$\text{}^{\dagger}$} & \textbf{91.50}\rlap{$\text{}^{\dagger}$} & \textbf{87.12}\rlap{$\text{}^{\dagger}$}	& \textbf{61.97}\\\hline
\end{tabular}
}
\caption{Overall Performance of RAG Models Optimized Using Different Judgment Models. The \textbf{best} result is highlighted. $\text{}^{\dagger}$ indicates statistically significant improvements over the Raw Metric model.}
\label{table1:overall}
\end{table*}

==> table/traindataset.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{l|r|r|r}
\hline
\textbf{Dataset} & \textbf{Total} & \textbf{Train} & \textbf{Dev}\\
% \hline
% \rowcolor{gray!8}\multicolumn{4}{l}{\textit{Training Judge Data}}\\
\hline
FinQA~\shortcite{chen2021finqa} &4,000 &3,800 &200\\
FiQA~\shortcite{maia201818} & 8,000 &7,600 &400\\
MeDiaQA~\shortcite{suri2021mediaqa} & 2,000 &1,900 &100\\
PubMedQA~\shortcite{jin2019pubmedqa}& 2,000 &1,900 &100 \\
ScienceQA~\shortcite{lu2022learn} & 7,095 &6,740 &355\\
NQ~\shortcite{nq2019Kwiatkowski}& 4,000 & 3,800 & 200 \\
ELI5~\shortcite{fan-etal-2019-eli5} & 4,000 &3,800 &200\\
NarrativeQA~\shortcite{kovcisky2018narrativeqa} & 2,000 &1,900 &100 \\
PopQA~\shortcite{mallen2023not} & 14,267 &13,554 & 713\\
CNNSum~\shortcite{wei2024cnnsum} & 8,000 &7,600 &400\\
MuSiQue~\shortcite{trivedi2022musique} & 22,355 &21,237 &1,118\\
\hline
\end{tabular}
\caption{Statistics of Data Used for Training \method{}.}
\label{table1:traindataset}  % 设置表格的标签
\end{table}
